CLIPSwarm: Converting text into formations of robots

We present CLIPSwarm, an algorithm to generate robot swarm formations from natural language descriptions. CLIPSwarm receives an input text and finds the position of the robots to form a shape that corresponds to the given text. To do so, we implement a variation of the Montecarlo particle filter to obtain a matching formation iteratively. In every iteration, we generate a set of new formations and evaluate their Clip Similarity with the given text, selecting the best formations according to this metric. This metric is obtained using Clip, [1], an existing foundation model trained to encode images and texts into vectors within a common latent space. The comparison between these vectors determines how likely the given text describes the shapes. Our initial proof of concept shows the potential of this solution to generate robot swarm formations just from natural language descriptions and demonstrates a novel application of foundation models, such as CLIP, in the field of multi-robot systems. In this first approach, we create formations using a Convex-Hull approach. Next steps include more robust and generic representation and optimization steps in the process of obtaining a suitable swarm formation.

==> 02_Related_work.tex <==
%Artistic robotics
Artistic robotics is a relatively novel stream of research in robotics and is attracting the interest of both the general audience and the robotics community. There are a variety of streams included under the term \textit{'artistic robotics'}. For instance, some works explore the possibilities of converting a robot into a painter, with techniques that go from copying existing techniques from real painters \cite{scalera2019non, beltramello2020artistic}, preprocessing the input images to simplify the input given to the robot \cite{karimov2021image} or even  to paint graffiti autonomously, \cite{chen2022gtgraffiti}. In some works, the robots are able to sculpt sculptures without human interaction \cite{ma2021stylized}.

There exist more expressions of art beyond sculpture or painting. For instance, some solutions make the robots act as professional dancers~\cite{peng2015robotic} or autonomous cinematographers. In this last stream, the robots are able to record cinematographic scenes autonomously satisfying some artistic or technical details, \cite{bonatti2020autonomous, cinempc}.

%Formations with shapes
In the stream of multirobot 2D artistic robotic formations, there are works that focus on optimal control to move the robots forming a set of given patterns, \cite{alonso2011multi, alonso2012image}. The same authors incorporated an interface to draw the desired pattern in \cite{hauri2013multi}. More recent approaches address how to perform multidrone formations shows, \cite{waibel2017drone, kim2016realization, sun2020path}.

All these works receive the desired pattern as input. Nevertheless, in CineClip the users do not need to create the patterns beforehand and can give instructions in natural language to the system and the platform will automatically decide the best positions for the team of robots to represent the formation that is described by the text input.
